Tunable Trajectory Planner Using G3 Curves

Trajectory planning is commonly used as part of a local planner in autonomous driving. This paper considers the problem of planning a continuous-curvature-rate trajectory between fixed start and goal states that minimizes a tunable trade-off between passenger comfort and travel time. The problem is an instance of infinite dimensional optimization over two continuous functions: a path, and a velocity profile. We propose a simplification of this problem that facilitates the discretization of both functions. This paper also proposes a method to quickly generate minimal-length paths between start and goal states based on a single tuning parameter: the second derivative of curvature. Furthermore, we discretize the set of velocity profiles along a given path into a selection of acceleration way-points along the path. Gradient-descent is then employed to minimize cost over feasible choices of the second derivative of curvature, and acceleration way-points, resulting in a method that repeatedly solves the path and velocity profiles in an iterative fashion. Numerical examples are provided to illustrate the benefits of the proposed methods.

==> name.tex <==
\section{Approximating Cubic Fresnel Integrals}
% the \\ insures the section title is centered below the phrase: AppendixA
We now address the problem of computing a general cubic Fresnel integral.  Let [CITE SOMETHING]
$$
P(s)=\int_0^s \cos\left(\frac{\pi}{2}u^2\right)du, \ S(s)=\int_0^s \sin\left(\frac{\pi}{2}u^2\right)du,
$$
denote the quadratic cosine and sine Fresnel integrals (resp.).  We generalize these integrals to polynomials of degree $n$, and between arbitrary start and goal arc-lengths as follows:
\begin{equation}
    \begin{split}
        P(P^n(s), a, b) = \int_{a}^{b}\cos(P^{n}(u))du\\
        S(P^n(s), a, b) = \int_{a}^{b}\sin(P^{n}(u))du
    \end{split}
\end{equation}
for given values of $a,b$, and where 
$$
P^n(s)=p_0+p_1s+\dots+p_ns^n.
$$
for $p_n\geq 0$.  We observe a useful identity that applies when $n=2$:
\begin{equation}
\begin{split}
\label{quad_ID}
    P^2(s)&=p_0+p_1s+p_2s^2\\
    &=e(s-v)^2+f \ \text{where},\\
    &e=p_2, \ v=-\frac{p_1}{2p_2}, \ f=p_0 - \frac{p_1^2}{4p_2}.
\end{split}
\end{equation}
Thus, 
\begin{equation}
\label{Csmid}
    \begin{split}
     P(P^2(s), s_1, s_2)=&\int_{s_1}^{s_2}\cos(e(u-v)^2+f)du\\
     =&\cos(f)\int_{s_1}^{s_2}\cos(e(u-v)^2)du \\ &-\sin(f)\int_{s_1}^{s_2}\sin(e(u-v)^2)du
    \end{split}
\end{equation}
Letting $m=\sqrt{2e/\pi}$, we observe that $m\in\mathbb{R}$ as $b_2\geq 0$ by assumption. We observe further, that using the substitution $e(u-v)^2=\pi r^2/2$, the equation \ref{Csmid} reduces to
\begin{equation}
    \label{Cq}
    \begin{split}
        &P(P^2(s), s_1, s_2)=\\
        &\frac{\cos(f)}{m}\left(P(m(s_2-v))-P(m(s_1-v)\right)\\
        &-\frac{\sin(f)}{m}\left(S(m(s_2-v))-S(m(s_1-v)\right).
    \end{split}
    \end{equation}
    Similarly,
 \begin{equation}
 \label{Sq}
    \begin{split}
        &S(P^2(s), s_1, s_2)=\\
        &\frac{\sin(f)}{m}\left(P(m(s_2-v))-P(m(s_1-v)\right)\\
        &+\frac{\cos(f)}{m}\left(S(m(s_2-v))-S(m(s_1-v)\right).
    \end{split}   
    \end{equation}
Equations~\eqref{Cq} and~\eqref{Sq} are used extensively in~\cite{1362698} to derive an analytic expression for the required curvature rate of a clothoid curve passing between start and goal configurations whose initial and final curvatures are 0.  It is suggested in~\cite{banzhaf2018g} that a similar approach to that in~\cite{1362698} can be employed to evaluate cubic Fresnel integrals $P(P^3(s), s_1, s_2), S(P^3(s), s_1, s_2)$.  However, this is cannot be done using a realtionship...bla bla bla


\begin{lemma}
\label{lem: cube to quad}
The cubic polynomial $P^3(s)=p_0+p_1s+p_2s^2+p_3s^3$ evaluated on the interval $[a, b]$ can be approximated using the quadratic polynomial 
\be
\label{cubetoquad}
\begin{split}
P_{\text{approx}}(s)&=p_0'+p_1's+p_2's^2, \ \text{where}\\
p_0' &= \frac{ab(a+b)p_3}{2}+p_0\\
p_1'&=-\frac{(a^2+4ab+b^2)p_3}{2}+p_1\\
p_2'&=\frac{3(a+b)p_3}{2}+p_2
\end{split}
\ee
with a maximum error of
\be
\label{maxer}
\max_{s\in[s_1, s_2]}|P^3(s)-P_{\text{approx}}(s)|=\frac{\sqrt{3}p_3}{36}(b-a)^3.
\ee
Furthermore, $P_{\text{approx}}(a)=P^{3}(a), P_{\text{approx}}(b)=P^{3}(b)$.
\end{lemma}
The proof of the lemma is omitted, but can be easily derived by replacing~\ref{cubetoquad} in \eqref{maxer}, and maximizing over $s\in[s_1, s_2]$. The values of $p_0', p_1', p_2'$ were computed by minimizing the squared error at the midpoint between $a$ and $b$.  That is,
\be
\begin{split}
\min_{p_0', p_1', p_2'} &\left(P^3\left(\frac{a+b}{2}\right)-P_{\text{approx}}\left(\frac{a+b}{2}\right)\right)^2\\
s.t. \ P^3(a)&=P_{\text{approx}}(a)\\
P^3(b)&=P_{\text{approx}}(b)
\end{split}
\ee
Suppose now that we wish to evaluate $P(P^3(s), a, b)$ to within a specified error $\epsilon$. To this end, we split $[a,b]$ into $k$ sub-intervals $[s_{i}, s_{i+1}]$ of equal length where $s_1=a, s_{k+1}=b$.  We observe that by Lemma \ref{lem: cube to quad}, we can approximate $P^3_i(s)$ on the sub-interval $[s_i, s_{i+1}]$ using a quadratic polynomial $P_{i, \text{approx}}=a_0^{i}+a_1^{i}+a_2^{i}$ using \eqref{cubetoquad} with a maximum error of 
$$
\frac{\sqrt{3}b_3}{36}(s_{i+1}-s_i)^3.
$$

Let 
$$
P_{i, \text{approx}}(s)=p_{i,0}'+p_{i,1}'s+p_{i,2}'s^2
$$
where $p_{i,j}', j=0,\dots,2$ are given by \eqref{cubetoquad} to approximate $P^3(s)$ on the interval $[s_i, s_{i+1}]$.  Similar to \eqref{quad_ID}, let
\begin{equation*}
\begin{split}
    e_i&=p_{i,2}', \ v_i=-\frac{p_{i,1}'}{2p_{i,2}'}\\
    f_i&=p_{i,0}'-\frac{(p_{i,1}')^2}{4p_{i,2}'}, m_i=\sqrt{\frac{2e_i}{\pi}}
\end{split}
\end{equation*}
Then by equations \eqref{Cq}, \eqref{Sq},
\be
\begin{split}
P(P^3(s), s_1, s_2)=& \sum_{i=0}^k\int_{s_i}^{s_{i+1}}\cos(P^3(u))du\\
\approx& \sum_{i=0}^k \int_{s_i}^{s_{i+1}}\cos(P_{i, \text{approx}}(u))du\\
S(P^3(s), s_1, s_2)=& \sum_{i=0}^k\int_{s_i}^{s_{i+1}}\cos(P^3(u))du\\
\approx& \sum_{i=0}^k \int_{s_i}^{s_{i+1}}\cos(S_{i, \text{approx}}(u))du
\end{split}
\ee
The integrals between $s_i$ and $s_{i+1}$ can now be evaluated using \eqref{Cq}, \eqref{Sq} as $P_{i,\text{approx}}(s)$ are quadratic functions of $s$ for each $i=1,\dots,k$.   An analytic approximation of $P(s), S(s)$ is provided in the appendix.
\end{proof}


\section{Work}
\begin{equation}
\begin{split}
C&=\int_0^{t_f}\mathcal{L}(\vect{w}, C_a, C_{\J}, C_y)dt\\
&\mathcal{L}(\vect{w}, C_a, C_{\J}, C_y)= w_a\left(\left(\ka v^2\right)^2+a_T^2\right) \\
&+ w_{\J}\left(\left(2va\ka + v^3\sigma\right)^2 + \left(a_T'\right)^2\right)\\
&+w_y(\ka v)^2 + w_t
\end{split}
\end{equation}
We make the following change of variables:

\begin{align*}
&y_1= \ka v^2,  &&y_2 = 2va_T \ka +v^3 \sigma\\
&y_3 =  a_T,  &&u = a_T'\\
&y_4 = \theta,  &&y_5 = \ka v    
\end{align*}
Letting $\vect{y}=[y_1 \dots y_5]^T$, we observe that we may re-write the cost as
\begin{equation}
 \int_{0}^{t_f}\vect{y}^TQ\vect{y} + Ru^2 dt
\end{equation}

$$
\nabla_{xx}^2
$$


\begin{equation}
    \begin{split}
    y_1' = y_2\\
    y_2' = 
    \end{split}
\end{equation}
